ScaMaha: A Tool for Parsing, Analyzing, and Visualizing Object-Oriented Software Systems

Reverse engineering tools are required to handle the complexity of software products and the unique requirements of many different tasks, like software analysis and visualization. Thus, reverse engineering tools should adapt to a variety of cases. Static Code Analysis (SCA) is a technique for analyzing and exploring software source code without running it. Manual review of software source code puts additional effort on software developers and is a tedious, error-prone, and costly job. This paper proposes an original approach (called ScaMaha) for Object-Oriented (OO) source code analysis and visualization based on SCA. ScaMaha is a modular, flexible, and extensible reverse engineering tool. ScaMaha revolves around a new meta-model and a new code parser, analyzer, and visualizer. ScaMaha parser extracts software source code based on the Abstract Syntax Tree (AST) and stores this code as a code file. The code file includes all software code identifiers, relations, and structural information. ScaMaha analyzer studies and exploits the code files to generate useful information regarding software source code. The software metrics file gives unique metrics regarding software systems, such as the number of method access relations. Software source code visualization plays an important role in software comprehension. Thus, ScaMaha visualizer exploits code files to visualize different aspects of software source code. The visualizer generates unique graphs about software source code, like the visualization of inheritance relations. ScaMaha tool was applied to several case studies from small to large software systems, such as drawing shapes, mobile photo, health watcher, rhino, and ArgoUML. Results show the scalability, performance, soundness, and accuracy of ScaMaha tool. Evaluation metrics, such as precision and recall, demonstrate the accuracy of ScaMaha ...

==> ijcds_biographies.tex <==
\vspace{-.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{figures/rafat}\squeezeup}]
{Ra'Fat Al-Msie'Deen} has been a Full Professor of Computer Science at Mutah University in Al-Karak, Jordan, since 2014. He received his PhD in Software Engineering from the Université de Montpellier, Montpellier - France, in 2014. He received his MSc in Information Technology from the University Utara Malaysia, Kedah - Malaysia, in 2009. He got his BSc in Computer Science from Al-Hussein Bin Talal University, Ma'an - Jordan, in 2007. His research interests include software engineering, requirements engineering, software product line engineering, feature identification, word clouds, and formal concept analysis. Dr. Al-Msie'Deen aimed to utilize his background and skills in the academic and professional fields to enhance students expertise in developing software systems. Contact him at \href{mailto:rafatalmsiedeen@mutah.edu.jo}{\faEnvelope}\href{mailto:rafatalmsiedeen@mutah.edu.jo}{ rafatalmsiedeen@mutah.edu.jo}. Also, you can reach him using different alternatives: \href{https://rafat66.github.io/Al-Msie-Deen/}{\faGithub}\href{https://rafat66.github.io/Al-Msie-Deen/}{ author's page @ github.io}, \href{https://www.linkedin.com/in/ra-fat-al-msie-deen-83a067314/}{\faLinkedin}\href{https://www.linkedin.com/in/ra-fat-al-msie-deen-83a067314/}{ LinkedIn}, \href{https://www.researchgate.net/profile/Rafat-Al-Msiedeen}{\includegraphics[width=0.022\textwidth]{figures/rG.png}}\href{https://www.researchgate.net/profile/Rafat-Al-Msiedeen}{ ResearchGate}, or \href{https://orcid.org/0000-0002-9559-2293}{\includegraphics[width=0.022\textwidth]{figures/iD.png}}\href{https://orcid.org/0000-0002-9559-2293}{ Orcid}.
\end{IEEEbiography}

